Quasi Anomalous Knowledge: Searching for new physics with embedded knowledge

Discoveries of new phenomena often involve a dedicated search for a hypothetical physics signature. Recently, novel deep learning techniques have emerged for anomaly detection in the absence of a signal prior. However, by ignoring signal priors, the sensitivity of these approaches is significantly reduced. We present a new strategy dubbed Quasi Anomalous Knowledge (QUAK), whereby we introduce alternative signal priors that capture some of the salient features of new physics signatures, allowing for the recovery of sensitivity even when the alternative signal is incorrect. This approach can be applied to a broad range of physics models and neural network architectures. In this paper, we apply QUAK to anomaly detection of new physics events at the CERN Large Hadron Collider utilizing variational autoencoders with normalizing flow.

==> intro.tex <==

in the LHC setting there was a go

Howeverm the accuracy of MC samples are litmited  
they will always be approximate priors 

and for the BSM physics, we iwll never have accurate prior,   ( but we have belief that they will resemble known physics ) 


In the absence of label

Unsupervised learning allows us to do density estimation by training only on data without labels. 


The typical anomaly detection with unsupervised learning involves following steps. Train the model with known background or normal events, and train the model so that it learns manifold of normal data. 

We propose a 

approximate or pseudo prior which 


The introduction(Use) of approximate priors allows us to add another dimension to the




In the following section, we will demonstrate the method in various different settings. 




ROC curve,  sensitivity efficiency curve, p-r curve





Architecture - NF VAE
there has been effort to use NF for anomaly detection (Andrey Ustuyashin) 

==> introduction_old.tex <==
With no evidence for new physical phenomena, many physicists at the Large Hadron Collider (LHC) are asking themselves a critical question: \emph{Am I searching for new physics in the right way?} This question has historically been  interesting. With incredible amounts of data at the LHC, a rapidly growing cohort is becoming concerned that we have somehow missed a new fundamental physics discovery.

Traditional searches for new physics at the LHC consist of three specific aspects:
\begin{itemize} 
\item an event selection:  a set of events are selected based on specific features,
\item a discriminator  : a variable that discriminates between a hypothesized signal against predicted backgrounds, and
\item a sensitivity estimate : a strategy to model the background shape of the discriminating variable.
\end{itemize}

The critical aspect of searches is that one constructs the selection, discriminator, and sensitivity estimate under a prior for what we think the signal model will look like. As an example, consider a search for black holes.  First, we hypothesize what a black hole signature would look like. From our hypothesis, we construct a Monte Carlo simulation of black hole signal events. We proceed to build an analysis around the assumption that we are searching for black holes. Barring a discovery, our final search will give us bounds on the production of black hole processes under these assumptions. It may not give us a bound on any other process; it might not even cover all possible black hole signatures. However, it will have shown that, in the region of collision data where events are black hole like, we observe good modeling of predicted background processes with the data. While the choice of a specific signal signature has been restrictive, it has the benefit that, for physics models that would have looked like our signal, we can make very strong constraints. 

To search broadly for new physics, the strategy at the LHC over the past 10 years or operation has been to write a very large list of possible new physics signal hypotheses and to iteratively go through this list and test to see if such a signal hypothesis is true. The large size of LHC experiments, with thousands of members, the large amounts of data and the very effective simulation tools have allowed us to streamline this process to achieve many 1000s of exclusions on possible new physics models. Despite the many exclusions, it seems that there is an endless limit of physics models yielding a seemingly unlimited number of possibilities. As an example, following an excess that was observed by both major collaborations at the LHC in 2015\cite{Khachatryan:2016hje,Aaboud:2016tru} more than 500 separate explanations of this new phenomenon were published. While it is fantastic that we have such powerful tools, it eliminates the intuition that has guided new physics searches at the LHC. We are left with the daunting option of trying to search for a new physics signature in every piece of data. 

%Start here
An alternative approach to a search for a new physics model is to search for anomalies in the data. Effectively, this means removing the new physics statistical prior  and instead of searching for events that are not like the predicted background. The idea to perform signal free searches, traditionally referred to as model-independent searches have been attempted on several occasions over the past two decades~\cite{PhysRevD.62.092004,PhysRevD.64.012004,PhysRevLett.86.3712,AKTAS200414,Wessels:2007md,Aaltonen:2007dg,Aaltonen:2007ab,Aaltonen:2008vt,CMS-PAS-EXO-14-016,Aaboud:2018ufy}. In general, these approaches have had limited success due to (1) the lack of sensitivity when compared with dedicated searches, (2) limited computing ability to probe all possible final states, (3) standard model background simulation that is imperfect, and (4) a general feeling that new physics had to have a clear cut signal. With the large amount of data, the rise of machine learning, improved background simulation, and frustration for not having found new physics by conventional means, a small group of the high energy physics community is coming back to these model independent search strategies and trying to investigate whether we now have the toolset to perform effective model independent searches that can have a lasting impact~\cite{Metodiev:2017vrx,Nachman:2020lpy,Andreassen:2020nkr,Collins:2018epr,Collins:2019jip,Farina:2018fyg,Heimel:2018mkt}.  %In light of these developments, a data challenge, know as the LHC Olympics has been organized, to assess the feasibility of different strategies and motivate future ideas.

In constructing model-independent searches a strong emphasis has been placed on the absence of a signal prior. Excluding a signal prior helps to ensure model independence. The exclusion of a signal prior then leads to the development of approaches that aim to model the standard model with progressively higher precision. New physics is then classified as an anomalous deviation from the observed standard model data distribution. This approach largely covers the class of analyses that use deep learning based anomaly detection consisting of either an autoencoder, variational autoencoder, normalizing flow algorithm or an adversarial network. Another class of anomaly detection insert a prior that the signal can be localized within a specific distribution. This prior allows for a weakly supervised training approach whereby one trains one region of data against another region. Provided that the observed differences within the background are completely understood, deviations on top of this training result in anomalies\cite{}. This second approach, often referred to as classification with out labels (CWOLA) can provide enhanced discrimination power over a bare autoencoder approach. This enhanced discrimination power largely results from the addition of a signal prior, in this case a signal localized in a specific kinematic regime. In this paper, we aim to further enhance the importance of signal priors by inserting additional signal priors into the search. By inserting additional signal priors through a ssytematic way, we aim to preserve the model independence, and to enhance the sensitivity towards signals with specific priors. Since, we systematically add priors, we inject information that can be viewed as Quasi-Anamalous Knowledge, or simply QUAK.

With QUAK, we propose a mechanism to allow for the interpolation between a search for new physics where a signal hypothesis is used to a search for new physics  where no signal hypothesis is used. For many classes of new physics models, there is a broad set of underlying physics features we can assume about any new signal; one such example is Lorentz invariance or the assumption that all particles from a massive object fall within a cone. Another such assumpition is the absence of color flow. With QUAK, we aim to embed these assumptions into our search while still preserving the model-independence of the search. To perform this we will rely on semi-supervised approaches applized to normalizing flow, and variational auto-encoders. While the exact deep learning architecture is not critical, we focus on  normalizing flow, since it most closely represents the physical models\cite{}. 

As a baseline for our studies, we first show the performance on the MNIST dataset. Here, the goal is to show the generality of the approach, since it can be applied to a broad range of models. Secondly, we QUAK the LHC Olympic challenge. The LHC Olympic challenge started in the fall of 2019. The challenge is focused on finding anomalies originating from an anomalous di-jet pair where one or two of the jets and the pair are anomalous. In the LHC Olympics, three unknown "black box" datasets, are prepared with a signal that is injected at a small rate within the data. A background simulation sample and signal simulation sample are also provided to allow for the training and testing of algorithms. The simulation signal is different from the actual secret hidden signal in the black box dataset and the background simulation is different than the black box dataset to mimic the fact that background simulations do not agree perfectly with data. The signal model for the first black box in the challenge was revealed at the ML4Jets conference in Jan 2020\cite{}.


==> simulation.tex <==
For the simulation, we use 

==> strategy.tex <==

\subsection{General description}


With QUAK (QUAsi-Anomalous Knowledge) we try to introduce approximate priors into the search of BSM physics, by injecting our belief about properties of BSM physics that should be preserved. We can inject multiple beliefs, and the belief doesn't have to be completely accurate. Approximate priors encode our belief about what the BSM model should preserve. 

There has been a number of ideas on how to do anomaly detection (tnt, anode ..) to search for Beyond the Standard Model physics in the context of dijet anomaly search. 

Here we present a general framework for doing anomalous jet tagging or anomaly detection or studying anomalous decay of particles 

The application is numerous, and not limited to specific model or anomaly metric. 

Where we incorporate aspsects of known physics that BSM model should have such as color flow, lorentz invariance, resonance formation ... etc. We are free to add any number of priors to the QUAK method. 

To do this in practice, in QUAK method framework, we train N number of probabilistic models for N number of priors we want to incorporate into the search. With these N priors incorporated to our search, we choose an anomaly metric that measures the typicality of the data seen at test time with the i th prior used for training. Therefore using the n sets of anomaly scores, we perform the search. 

Any probabilistic model is possible, GAN ,...
To test this idea, the studies were done with the MNIST dataset, and the official LHC Olympics 2020 anomaly detection dataset.  

\subsection{LHCO study setup}

The studies presented here were done on the official LHC Olympics 2020 dataset \cite{kasieczka_gregor_2019_3596919}, and samples generated using the same parameters as in LHCO 2020 dataset with the help of the organizers. The BSM events in the dataset are dijet events from BSM resonances with the same decay mode X->YZ, characterized by the mass of the resonance X represented by the dijet mass mjj, mass of decay products Y and Z which decays hadronically and reconstructed as jets $m_{j1}$ and $m_{j2}$, and decay modes of the particles Y and Z, which is denoted as n prong (for Y -> n quarks). We generated variety of samples with different dijet mass, jet 1 and jet 2 jet masses, and 2 different decay modes (2 prong decay and 3 prong decay). 

We use higher level jet features as our input, namely n-subjettines jet massses in the individual jets. 
Studies were performed with 12 sets of variables as used in \cite{Nachman_2020} and \cite{Metodiev_2017}.

\begin{equation}
\label{eqn:features}
  \{m_{jj},m_{j1}, j1 \tau_{21}, j1 \tau_{32}, j1 \tau_{43}, m_{j2} , j3, j4\}
\end{equation}

%Instead of doing n dimensional scan, we can just empirically choose a working point. 

The probabilistic model we chose for the studies with the LHC Olympics dataset are variational autoencoders (VAEs) with normalizing flows \cite{rezende2015variational} for better posterior approximation. We tried a variety of flow architectures that are out in the market, and its performance in the context of LHCO data is tabulated in table X. Based on table X, We chose Masked Autoregressive Flow as our flow architecture, \cite{papamakarios2017masked} described in the previous chapter\cite{}.


\subsection{model selection and model parameter scan}

We also scanned beta value from a $\beta$ - vae paper 

described in \cite{Higgins2017betaVAELB}, which is a 
with beta value that scales the KL divergence term with 10.0. Beta parameter optimization was also performed, and the AUROC result is tabulated in table x. 

The anomaly metric was chosen as the reconstruction loss of the testing data. We use reconstruction loss (or any measure of likelihood) of each test event, but any measure of typicality, such as distance measure such as Earth Mover's distance in collider events could also be used as a metric in QUAK method. 

As it was described earlier about QUAK, we first train 1

First we do a comparioson of 1D, 2D and 3D QUAK, 

Supervised architecture: fully connected with batchnorm and dropout
Unsupervised : learnable mapping fully connected
include diagram


 


We observe that supervised classifiers we build perform gradually worse , and it performs badly especially when we change the decay mode of each jets( from two-prong decay into three-prong decay. 




In Fig. X, we compare the performance of supervised classifier and QUAK method. 




Thus we learn that using QUAK allows us to incorporate signal priors into the search.
Anomaly detection in the context of searching for BSM physics, where incorporate prior knowledge about,, encode our belief that BSM physics should have some aspect which resembles the known physics,  injet signal occasional input from 






\begin{figure}[htbp]
\centering
\includegraphics[width=.45\linewidth]{images/plot1_2prongtest.png}
\includegraphics[width=.45\linewidth]{images/plot1_3prongtest.png}
    \caption{(Left) Receiver Operator Characteristic (ROC) for signal versus background selection for various algorithms. 
    
    
    
    Here, we  care about the dashed lines when either the correct (blue-dashed) or incorrect (red-dashed) signals are used to discriminate against the background. The solid lines represent the performance of individual discriminators for background only, signal, and incorrect signal. (Right) The result of using the first iteration of QUASAR on the LHC Olympic dataset to find a hidden signal. The red line corresponds to where the hidden signal is expected to peak.  
    
    
    
    }
       \label{fig:qaperf}
\end{figure}



We are trying to show that you can add N number of priors for QUAK method to get performance improvement

in 




Does it preserve the model independence of the search? Fig 3 shows that 

Intuitively we see that BSM events are more typical to known physics than QCD events. 


from the N unsupervised models and scan the 




First we see compare the sensitivity of 1D, 2D and 3D QUAK, which corresponds to using 1 prior ( QCD prior) , 2 priors (QCD and 2prong prior with (mjj,j1,j2) = ) and 3 priors (QCD prior and 2prong prior (mjj, 


We get N sets of losses from N models, After we build N dimensional space of losses we did the iterative scan of that loss 
$O^(n)$
More effective way to such as using linear discriminator to 



First we show that adding priors improve the sensitivity of the search. 
adding relevant prior boosts performance more
even adding wrong prior helps a lot 




For QUAK, 

we consider building two separate normalizing flow neural networks, one network on signal sample A and one network on background B. 





With these networks, we aim to search for anomalies concerning both A and B.  Normalizing flow networks are a class of neural networks that aim to build a physical space that model the information needed to train the deep neural network\cite{2015arXiv150505770J}; they are found to be very effective at solving complicated physics problems\cite{2020arXiv200202428J}. 




QUAK provides a nice way to inject priors into the search of possible BSM models. Similar thing can be done by training an appropriate supervised model. 

Supervised model learns the decision boundary of the model, and when tested on a test data with significantly different

QUAK is more stable when the prior changes (but is still significantly different from the QCD prior), but still is anomalous. If we think of injecting priors meaning they occupy some space in the latent space and we measure the distance measure between them and the 

Training a generative model and getting the loss gives us the sense of distance metric between two priors. 
For QUAK framework, any generative neural network works


We also compare different VAE architectures and also compare the performance of different flow architectures. 

%n dimensional prior space, use set notation
\begin{table}[ht]
\caption{AUC for different \beta-parameters} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
\beta & Background Prior & Signal  Correct Prior & Signal Prior (on wrong prior) \\ [0.5ex] % inserts table
%heading

\hline % inserts single horizontal line
0.1 & 0.771 & 0.939 & 0.628 \\ % inserting body of the table
0.5 & 0.774 & 0.972 & 0.700 \\
1.0 & 0.775 & 0.977 & 0.796 \\
2.0 & 0.803 & 0.981 & 0.799 \\
10.0 & 0.840 & 0.983 & 0.831 \\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:betascan} % is used to refer this table in the text
\end{table}


The model was chosen to be 
and the model parameter scan for different beta values was performed and result is tabulated in table \ref{table:betascan}


With the construction of new anomalous discriminators, we can build a space where events are \emph{not} signal anomalies, but \emph{are} background anomalies. With this space, we can construct a signal discriminator to separate A from B. Additionally if signal events are like A, but not exactly A, they will end up in this space in a region of low anomaly with respect to A but still be anomalous to B. In this way, we can use the same discriminator construction to search for signals even when the signal A is incorrect. 

To illustrate this idea, using the LHC Olympic dataset, we constructed a modified signal set by taking a known signal and removing events that had a characteristic signal feature.  We then constructed a discriminator with this modified signal and we compare it to the performance when the signal was fully correct. 



This is shown in the left plot of figure~\ref{fig:qaperf}. What we observe is that while we are unable to capture the full performance of the best discriminator, we are capable of getting close despite the signal model being incorrect. 




We further tested this idea on the LHC Olympic dataset using the first black box. Despite not knowing the signal, we were able to build a discriminator for signal against the background. By cutting on this discriminator, we were able to obtain the right plot in figure~\ref{fig:qaperf} where we observe an excess of blue events over our background prediction in red. This excess turns out to be right at the true signal of the black box, which is indicated by the red line. These plots are the first proof of concept that QUASAR will work. It should be noted that in Jan 2020, when the first black box was revealed only 2 out of 10 submissions were able to observe the correct signal excess.  While our proof of concept demonstration is not yet published,  it is sufficient to continue our work towards publication in the summer. 


Comparison with the fully supervised classifier is also shown as reference. 


\begin{figure}[htbp]
\centering
\includegraphics[width=1.\linewidth]{images/plot2_combined.png}
    \caption{(Left) Receiver Operator Characteristic (ROC) for signal versus background selection for various algorithms. Solid lines represent the supervised classifier trained on (mjj, mj1, mj2) = (4500,500,150) tested with a variety of BSM models with different mass and decay mode. 
    
    
    
    Here, we  care about the dashed lines when either the correct (blue-dashed) or incorrect (red-dashed) signals are used to discriminate against the background. The solid lines represent the performance of individual discriminators for background only, signal, and incorrect signal. (Right) The result of using the first iteration of QUASAR on the LHC Olympic dataset to find a hidden signal. The red line corresponds to where the hidden signal is expected to peak.  }
       \label{fig:qaperf}
\end{figure}


Here we compare 2D QUAK with supervised classifier trained with same raw inputs and same signal prior used for QUAK classifier. We observe the general trend that supervised classifier performs gradually worse as the test data deviates further from the prior that was used to train the classifier, and performs really badly when we change the decay mode. On the other hand we observe that QUAK method performs relatively stable as the prior deviates from the priors included in the training. This allows QUAK to do more efficient scan of the entire BSM space than just using supervised classifiers. QUAK incorporates signal prior in a more efficient way than supervised classifiers. However, we observe that for 2D QUAK, Decision boundary and learning the structure of data, therefore it behaves more stable. 



\begin{figure}[htbp]
\centering
\includegraphics[width=1.\linewidth]{images/plot3_combined.png}
    \caption{(Left) Receiver Operator Characteristic (ROC) for signal versus background selection for various algorithms. Solid lines represent the supervised classifier trained on (mjj, mj1, mj2) = (4500,500,150) tested with a variety of BSM models with different mass and decay mode. Here, we  care about the dashed lines when either the correct (blue-dashed) or incorrect (red-dashed) signals are used to discriminate against the background. The solid lines represent the performance of individual discriminators for background only, signal, and incorrect signal. (Right) The result of using the first iteration of QUASAR on the LHC Olympic dataset to find a hidden signal. The red line corresponds to where the hidden signal is expected to peak.  }
    \label{fig:qaperf}
\end{figure}


Last plot shows the reverse of what was done in plot 2. Here we include different priors for QUAK



With more work, we can further improve the quality of QUASAR. In particular, we are looking at deep learning approaches to impose Lorentz invariance and other fundamental physical symmetries in the network. 

Additionally, we are working to extend the scope of deep learning by exploring some of the newer normalizing flow approaches including real value non volume preserving flow. 

Lastly, through variational approaches, we would like to embed uncertainties into this approach to quantify the significance of our anomalies. 


Beyond the LHC Olympics, we plan to use this algorithm as a tool to perform searches over a broad set of signals where most of the signals, but not all of the signals are known. In particular, we would like to apply this to the problem of characterizing all the anomalous decays of the Higgs boson. We believe that this approach can be used as a way to bound anomalous decays of the Higgs boson since all such decays have a class of distinct features. With QUASAR, we believe we can capture the common features universal to  a Higgs boson decay while simultaneously searching for all possible Higgs boson decays. Even a partial bound on Higgs decay final states will have profound implications on the fundamental nature of physics models and can lead to a fundamental measurement of the Higgs boson's properties~\cite{Harris:2019qwx}.   %Lastly, we also see that, with QUASAR, we can start to classify anomalous events by their properties. This can be very useful when we are trying to characterize the different sources of noisy events at the LHC.  


We will call the data we add 
Signal priors refer to BSM model we add to the training that we believe 


Adding signal priors to anomaly loss 


allows for enhanced identification of anomalies by providing generic "signal-like" features to help in identification. This follows the ML paradigm of semi-supervised learning



Note on Interpretability: It is imoprtant to note that QUAK provides a nice iterative way to refine the search while helping with the sensitivity to a wide variety of different physics models. QUAK address the question of how do we interpret the signal we obtain nicely? QUAK is meant to help mostly with the search, because if the real signal has any resemblance to multiple priors we added to to the search then it will significantly improve the sensitivity of that search, and then we can study the selected events, and refine the search with the properties we observe from the selected sample  Iterative method (cite TNT) 
